Dolha - an Efficient and Exact Data Structure for Streaming Graphs

A streaming graph is a graph formed by a sequence of incoming edges with time stamps. Unlike static graphs, the streaming graph is highly dynamic and time related. In the real world, the high volume and velocity streaming graphs such as internet traffic data, social network communication data and financial transfer data are bringing challenges to the classic graph data structures. We present a new data structure: double orthogonal list in hash table (Dolha) which is a high speed and high memory efficiency graph structure applicable to streaming graph. Dolha has constant time cost for single edge and near linear space cost that we can contain billions of edges information in memory size and process an incoming edge in nanoseconds. Dolha also has linear time cost for neighborhood queries, which allow it to support most algorithms in graphs without extra cost. We also present a persistent structure based on Dolha that has the ability to handle the sliding window update and time related queries.

==> concluions.tex <==
%\vspace{-0.1in}
\section {Conclusions}
%\vspace{-0.05in}
\label{sec:con}
We have proposed an exact streaming graph structure Dolha which could maintain high speed and high volume streaming graph in linear time cost and near linear space cost. We have shown that Dolha is a general propose structure that could support the query primitives which are the cornerstone of common graph algorithms. We also present the Dolha persistent structure which could support sliding window update and time related queries. The experiment results have proved that Dolha has better performance than the other streaming graph structures.

==> dolhapersistent.tex <==
\section{Dolha Persistent Structure} \label{sec:baseline}
%\vspace{-0.05in}
\subsection{Dolha Persistent Data Structure}
Using Dolha, We could construct a persistent structure $D_p$ and $D_p$ contains any snapshot's information of $\iG$. $D_p$ has the same structure as $D_s$ except the time travel list.

\begin{definition}[Time Travel List]  \label{def:timetravellist}
	An edge $\overrightarrow {uv}$ may appear in streaming graph $S$ multiple times with different time stamp. Time travel list $T$ is a single linked list that links all the edges $\overrightarrow {uv}$ which share same outgoing and incoming vertices. In $T$, each edge has an index points to its previous appearance in the stream.
\end{definition}

$D_p$ also has four index-value tables. The vertex hash table, vertex table and edge hash table are same as $D_s$. In each cell of edge table, $D_p$ has a extra value \nop {$E^T_{P}(*)$} which indicates the previous item on the time travel list.

\subsection{Dolha Persistent Construction}
\subsubsection{Incoming Edge Processing}
When an edge $\sigma(\overrightarrow {uv};t;w)$ comes: 
\begin{itemize}
		\item
            Check the existence of $\overrightarrow {uv}$ same as Dolha snapshot.
	\end{itemize}


	 \textbf{If $\overrightarrow {uv}$ does not exist in $D_p$:}
	\begin{itemize}
		\item
            The operation is exact same as Dolha snapshot.
	\end{itemize}
		
	 \textbf{If $\overrightarrow {uv}$ exists in $D_p$:}
	\begin{itemize}
	    \item
	    Use edge hash table to find the existing edge table index $E(\sigma ')$ of $\overrightarrow {uv}$.
		\item
		    Insert edge $\sigma$ as new edge into edge table and set the time travel list index as $E(\sigma ')$.
		\item
		    Update the edge table index of $\overrightarrow {uv}$ on edge hash collision list. 
	\end{itemize}


    
\begin{algorithm}[h!]
\small
\caption{Dolha persistent edge processing}
    \label{alg:persistent}
\KwIn{Streaming graph $\iG$}
\KwOut{Dolha persistent structure of $\iG$}
\For{each incoming edge $\sigma(\overrightarrow {uv};t;w)$ of $\iG$}
{
    \textbf{Check existence of $\overrightarrow {uv}$:} \\
    \If{$\overrightarrow {uv}$ does not exist}
    {
        Insert $\overrightarrow {uv}$\\
    }
    \If{$\overrightarrow {uv}$ exists in cell $E(\sigma ')$}
    {
       Insert $E(\sigma)$ as new edge and let $w(\sigma)=w(\sigma)+w(\sigma ')$ \\
       Let $E^T_{P}(\sigma)=E(\sigma ')$\\
    }
    \If{value of $H(\overrightarrow {uv})$ in edge hash table is $null$}
    {
        Let $E^H_A(\overrightarrow {uv})=E(\sigma)$\\
    }
    \ELSE
    {
        Let $E^H_N(\overrightarrow {uv}^{-})=E(\sigma)$
    }
}	

\end{algorithm}

\nop{
\begin{table}[!h]
\centering
\small
    \caption{\mbred{Vertex table of Window 0}}     % NOTE!  caption goes _before_ the table contents !!
    \label{tab:vertextime}
	\resizebox{0.8\linewidth}{!}
	{
		\input{tab_vertextime}
	}
\end{table}
}
\begin{table}[!h]
\centering
\small
    \caption{\mbred{Edge hash table of Window 0}}     % NOTE!  caption goes _before_ the table contents !!
    \label{tab:edgetimehash}
	\resizebox{1\linewidth}{!}
	{
		\input{tab_edgetimehash}
	}
\end{table}

\begin{table}[!h]
\centering
\large
    \caption{\mbred{Edge table of Window 0}}     % NOTE!  caption goes _before_ the table contents !!
    \label{tab:edgetime}
	\resizebox{1.05\linewidth}{!}
	{
		\input{tab_edgetime}
	}
\end{table}

\begin{table}[!h]
\centering
\large
    \caption{\mbred{Edge table of Window 1}}     % NOTE!  caption goes _before_ the table contents !!
    \label{tab:edgewin1}
	\resizebox{1.05\linewidth}{!}
	{
		\input{tab_win1}
	}
\end{table}

Table \ref{tab:edgetimehash} and \ref{tab:edgetime} show the Dolha persistent's edge hash table and edge table of $\iG$ in Window 0. The vertex hash table and vertex table of  Dolha persistent are similar like Dolha snapshot and so is the new edge coming. But for edge $\overrightarrow{v_1v_2}$ update at time $6$, we add the update as new edge into $E(6)$ and update the edge hash table to latest update. By using the time travel list, all the updates of $\overrightarrow{v_1v_2}$ are linked. 

\subsubsection{Sliding Window Update}
When the window slides the $i$th step, we have the start time $t_s=t_0+(i-2) \times \theta$ and end time $t_e=t_0+(i-1) \times \theta$ of expired edges which need to delete from edge table. Since the edge table is naturally ordered by time, we can find the last expired edge denote as $E(\sigma_e)$ at $t_e$ in $O(\log S)$ time. By using edge hash table, we can find the latest update of $E(\sigma_\Omega)$ and traversal back by the time travel list. For each $E(\sigma_n) (e < n \le \Omega)$ on time travel list, let $w_n=w_n-w_e$. If each $w_n \le 0$, delete all the $E(\sigma_n)$. Then delete each $E(\sigma_m) (0 < m \le e)$ on time travel list. Do the same operation for the edges from $t_e$ to $t_s$. For every deleted edge, if it is the first or last item of Doll, update the associated cell in vertex table and set the index to $null$. If all the Doll indexes are $null$ in that vertex cell, delete the vertex and flag the cell as empty.

As shown in Figure \ref{fig:timewindow}, when window slides from $0$ to $1$ means the edges before $t_4$ will expire. First, we can binary search the edge table to locate the first unexpired edge index $3$ since the table is sorted by time stamp. Then we start to delete the expired edges from cell $3$. We use the hash table to check if there are unexpired updates for the expired edges. For example, $\overrightarrow{v_1v_2}$ has unexpired update at time $7$, so we minus the expired weight at cell $6$. 

Table \ref{tab:edgewin1} shows the edge table of Dolha persistent at Window 1. The first 3 expired edges have been deleted. At time $8$, $\overrightarrow{v_1v_4}$ with negative weight arrives, but there is no positive $\overrightarrow{v_1v_4}$ in this window. In this case, we won't save $\overrightarrow{v_1v_4}$. At time $9$ and $10$, $\overrightarrow{v_1v_2}$ has negative or zero weights, but $\overrightarrow{v_1v_4}$ has positive weight at time $7$, so we keep the record and link them with time travel linked list. 

\textbf{Space Recycle:} Due to the chronological ordered edge table, the expired edges are always continuous and in the head of the unexpired edges. We could always recycle the space from expired edges which means we won't need infinite space to save the continuous streaming but only need the maximum number of edges in each window. For instance, in table \ref{tab:edgewin1}, we can re-use the cell from $0$ to $1$ for next window update and we have enough space as long as no more than $9$ edges in $1$ window.



\subsection{Time and Space Cost}
The time cost of Dolha persistent is hash table cost, Doll cost and time travel list cost. For each incoming edge, the hash table cost and Doll cost are $O(1)$ as we discussed in Dolha snapshot and the time travel list cost is also $O(1)$ same as insertion on single linked list. Overall, the time cost for one edge processing is $O(1)$.

 To store all the information of streaming $S$, Dolha persistent structure needs one $|V|$ cells vertex hash table, one $|V|$ cells vertex table, one $|S|$ cells edge hash table and one $|S|$ cells edge table. In total, Dolha needs $(2 \times \log |V|+4 \times \log |S|) \times |V|+(2 \times \log |V|+5 \times \log |S|) \times |S|$ bits plus $\log |S| \times |S|$ for time travel list. The space cost of Dolha persistent structure is $O(|S|\log |S|)$. 


%in Appendix \ref{sec:appendix:pseudocodes}). 


